Contests to Incentivize a Target Group

We study how to incentivize agents in a target group to produce a higher output in the context of incomplete information, by means of rank-order allocation contests. We describe a symmetric Bayes--Nash equilibrium for contests that have two types of rank-based prizes: prizes that are accessible only to the agents in the target group; prizes that are accessible to everyone. We also specialize this equilibrium characterization to two important sub-cases: (i) contests that do not discriminate while awarding the prizes, i.e., only have prizes that are accessible to everyone; (ii) contests that have prize quotas for the groups, and each group can compete only for prizes in their share. For these models, we also study the properties of the contest that maximizes the expected total output by the agents in the target group.

==> aaai/conclude.tex <==
\section{Conclusion and Future Work}
% The development of underrepresented groups is integral to the progress of our society, and contests have been, and can be further, used to assist this goal. 
% Our work provides a theoretical framework to study such contests.
Our paper studies the equilibrium and the design of contests with rank-order allocation prizes that maximize the output of a target group.

An important open problem suggested by our work is understanding the properties of the optimal contest that has both group-specific and general prizes. We characterize the equilibrium for this problem and analyze the optimal contest for specific sub-cases, but the general problem is open. One possible way to make this tractable can be to assume large numbers of agents and prizes; such assumptions allow for a stronger and more tractable equilibrium characterization by making the influence of an individual agent infinitesimal~\cite{olszewski2016large}. 
Our work focused on contests with rank-order allocation of prizes with incomplete information and linear cost functions. %, but there are other good models to study contests that model real-life scenarios. For example, 
Instead of rank-order allocation of prizes, we can study proportional allocation of prizes or its generalizations (see, e.g., \citet{tullock1980efficient}); one motivation for proportional allocation is the randomness and unpredictability of outcome in the real world. Similarly, we may relax the assumption of linear cost functions, or we can study complete information models instead of incomplete information.

==> aaai/design.tex <==
\section{Designing Prizes to Incentivize the Target Group}\label{sec:des}
Based on the equilibrium characterizations in the previous section, in this section we investigate the properties of the optimal contest that maximizes the total output of the target group. We characterize the optimal contests for general prizes and for group-specific prizes only.

% If the contest designer wants to have only general prizes, to induce maximum output from the target group, she should divide the prize budget equally among top-$k$ ranked agents, where $k$ depends upon the relative frequency of the target group agents $\mu$ and the distributions $F$ and $G$. This result is proved in Theorem~\ref{thm:desGen} and uses the equilibrium characterization given in Theorem~\ref{thm:eqGen}. 
% This result is in contrast to maximizing total output of the entire population, where the entire prize should be allocated to the top-ranked agent~\cite{glazer1988optimal,moldovanu2001optimal}.

% If the designer wants only group-specific prizes, she should allocate the entire prize budget to the first prize, i.e., give a prize of $1$ to the top-ranked agent in the group; given in Theorem~\ref{thm:desTarget}. The proof of Theorem~\ref{thm:desTarget} extends the techniques used to provide a similar result for total output maximization~\cite{glazer1988optimal,moldovanu2001optimal}.

In the appendix, we compare the choice between only general and only group-specific prizes; we observe that either of them may be a better choice depending upon the situation. Even if the distributions of the target and the non-target group are the same, the relative frequency of target group agents, measured by $\mu$, determines which prize allocation scheme is better. If $\mu$ is sufficiently high, then it is better to have only group-specific prizes, while the converse is true if $\mu$ is very low. 






\subsection{General Prizes Only}\label{sec:desGen}
The strategy used by the agents in the target group is $\alpha(v)$, as derived in Theorem~\ref{thm:eqGen}. It can be rewritten as
\begin{align}
    \alpha(v) &= \sum_{j \in [n-1]} (w_j - w_{j+1}) \int_0^v y f^{\mu F + (1-\mu) G}_{n-1,j}(y) dy \nonumber \\
    &= \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^v y f^{\mu F + (1-\mu) G}_{n-1,j}(y) dy,
\end{align}
where $\gamma_j = j (w_j - w_{j+1})$. Instead of optimizing over $(w_j)_{j \in [n]}$, we can optimize over $(\gamma_j)_{j \in [n-1]}$ with constraints $\gamma_j \ge 0$ and $\sum_j \gamma_j = 1$, to find the optimal contest that maximizes the target group's output.

\begin{theorem}\label{thm:desGen}
The contest with general prizes only that maximizes the expected total output of the agents in the target group awards a prize of $1/k^*$ to the $k^*$ top-ranked agents and a prize of $0$ to the remaining $n-k^*$ agents, where $k^*$ is defined as
\[
    k^* \in \argmax_{j \in [n-1]} \langle \psi , f^{\mu F + (1-\mu) G}_{n,j+1} \rangle
\]
for $\psi(x) = \frac{x (1-F(x))}{1- \mu F(x) - (1-\mu) G(x)}$.
\end{theorem}

\begin{proof}
%[Proof of Theorem~\ref{thm:desGen}]
The expected output of an agent in the target group is $\bE_{v \sim F}[\alpha(v)]$, and maximizing this quantity maximizes the total output produced by all agents because $\mu$ and $n$ are constants. Let $H(v) = \mu F(v) + (1-\mu) G(v)$.
\begin{align*}
    &\bE_{v \sim F}[\alpha(v)] = \int_0^1 \alpha(v) dF(v) \\
    &= \int_0^1 \left( \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^v y f^{H}_{n-1,j}(y) dy \right) dF(v)\\
    &= \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^1 \left( \int_y^1 dF(v) \right) y f^{H}_{n-1,j}(y) dy \\ 
    &= \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^1 y (1-F(y)) f^{H}_{n-1,j}(y) dy. 
\end{align*}
As $\gamma_j \ge 0$ and $\sum_j \gamma_j = 1$, from the above expression we can observe that the optimal solution sets $\gamma_k > 0$ only if $\left(\frac{1}{j} \int_0^1 y (1-F(y)) f^{H}_{n-1,j}(y) dy \right)$ is maximized by $j = k$. Moreover, there is always an optimal solution where $\gamma_{k^*} = 1$ for some $k^* \in [n-1]$ and $\gamma_j = 0$ for $j \neq k^*$, where $k^*$ is given by:
\begin{align*}
    k^* &\in \argmax_{j \in [n-1]} \frac{1}{j} \int_0^1 y (1-F(y)) f^{H}_{n-1,j}(y) dy \\
    &= \argmax_{j \in [n-1]} \frac{1}{n} \int_0^1 y \frac{1-F(y)}{1-H(y)} f^{H}_{n,j+1}(y) dy \\
    &= \argmax_{j \in [n-1]} \langle \psi , f^{H}_{n,j+1}(y) \rangle,
\end{align*}
where $\psi(x) = x \frac{1-F(x)}{1-H(x)}$.
\end{proof}

Let $H(x)$ denote $\mu F(x) + (1-\mu) G(x)$. The function $\psi(x) = x\frac{1-F(x)}{1 - H(x)}$ in Theorem~\ref{thm:desGen} is independent of the prize structure: it depends only on $\mu$, $F$, and $G$, which are parameters given to the contest designer. The function $f^{H}_{n,j+1}(x)$ is the PDF of the $(j+1)$-th highest order statistic of the distribution $H$. The optimal $j = k^*$ maximizes the inner product between $\psi$ and $f^H_{n,j+1}$, and therefore, the similarity between them. In other words, the optimal $j = k^*$ selects the order statistic that is as similar to $\psi$ as possible.

Note that when we are maximizing the total output, then instead of an inner product of the order statistic with $\psi(x)$ in Theorem~\ref{thm:desGen}, we take an inner product with just $x$. As $x$ is monotonically increasing, the order statistic that is most similar to $x$ and that maximizes the inner product with $x$ is the one with $j = 1$, as shown by \citet{glazer1988optimal} and \citet{moldovanu2001optimal}. This provides an argument in favor of allocating the entire prize budget to the first prize. In contrast, when we focus on the target group only, it may be optimal to distribute the prize among several top-ranked agents. This also means that we may lose a portion of the total output, and this loss can be $\Omega(n)$ as shown in Example~\ref{ex:des:0}. Also, by the \textit{single-crossing} property, see \citet{vojnovic2015contest} Chapter 3, if we flatten the prize structure then we increase the output of the agents with low ability and decrease the output of the agents with high ability.

\begin{example}\label{ex:des:0}
Let $F(x) = 1 - (1-x)^{n-1}$, $G(x) = ((n-1)x - F(x))/(n-2)$, and $\mu = 1/(n-1)$. We get $H(x) = \mu F(x) + (1-\mu) G(x) = x$, which is the uniform distribution over $[0,1]$. Note that 
\[
    \psi(x) = \frac{x(1-F(x))}{1-H(x)} = \frac{x(1-x)^{n-1}}{(1-x)} = x(1-x)^{n-2}.
\]
It can be checked that the order-statistic that maximizes the inner-product with $\psi(x)$ is $f^H_{n,n-1}(x) = n(n-1)x(1-x)^{n-1}$. So, the optimal value is $k^* = n-2$. The total output generated for $k^* = n-2$ is
\begin{multline*}
    \frac{1}{n} \int_0^1 x f^{H}_{n,n-1}(x) dx \\
    = \frac{2}{n(n+1)} \int_0^1 f^{H}_{n+1,n-1}(x) dx = \frac{2}{n(n+1)}.
\end{multline*}
On the other hand, we know that the expected total output is maximized by $j=1$ and is equal to
\begin{multline*}
    \frac{1}{n} \int_0^1 x f^{H}_{n,2}(x) dx \\
    = \frac{(n-1)}{n(n+1)} \int_0^1 f^{H}_{n+1,2}(x) dx = \frac{(n-1)}{n(n+1)}.
\end{multline*}
The ratio between the two quantities is $(n-1)/2 = \Omega(n)$.
\end{example}

% Part of the longer calculations from the examples in this section are provided in the appendix.
% \begin{example}\label{ex:des:1}
% Let $F(x) = 2x-x^2$, $G(x) = x^2$, and $\mu = 1/2$. We get $H(x) = \mu F(x) + (1-\mu) G(x) = x$, which is the uniform distribution over $[0,1]$. We have:
% % \begin{equation*}
% % \frac{1}{j} \int_0^1 x (1-F(x)) h_{n-1,j}(x) dx = \frac{(n-j)(j+1)}{n(n+1)(n+2)}.
% % \end{equation*}
% \begin{align*}
%     \frac{1}{j} \int_0^1 x (1-F&(x)) h_{n-1,j}(x) dx \\
%     &= \frac{1}{j} \int_0^1 x (1-2x+x^2) h_{n-1,j}(x) dx \\
%     &= \frac{1}{j} \int_0^1 x (1-x)^2 h_{n-1,j}(x) dx \\
%     &= \frac{n-j}{j(n)} \int_0^1 (1-x)^2 h_{n,j}(x) dx \\
%     % &= \frac{n-j}{n(n+1)} \int_0^1 (1-x) h_{n+1,j+1}(x) dx \\
%     &= \frac{(n-j)(j+1)}{n(n+1)(n+2)} \int_0^1 h_{n+2,j+2}(x) dx \\
%     &= \frac{(n-j)(j+1)}{n(n+1)(n+2)}.
% \end{align*}
% Maximizing $\frac{(n-j)(j+1)}{n(n+1)(n+2)}$ w.r.t. $j$ is equivalent to maximizing $(n-j)(j+1)$. So, the optimal value is $k = \argmax_j (n-j)(j+1) = \lfloor \frac{n-1}{2} \rfloor \neq 1$ for large $n$.
% \end{example}

In the above example, the distribution of the target group $F$ was first-order stochastic (FOS) dominated by the distribution of the general population $H$.
% ; equivalently $F$ was FOS dominated by the distribution of the non-target group $G$. 
For this case, we observed that awarding prizes to more than one agent increases the expected output of the target group. $F$ being FOS dominated by $H$ means that the agents in the target group have lower ability than the general population. As flattening the prize structure increases the output of the lower ability agents and decreases the output of the higher ability agents, it makes sense that having a flatter prize structure incentivizes them.

The above result raises the question: What if the target group is equally able or stronger than the general population, i.e., if the distribution of the ability of an agent in the target group, $F$, FOS dominates the distribution of the ability of an agent in the non-target group, $G$; is it then optimal to award the full prize to the top-ranked agent? When $F = G = H$, we know that it is optimal to give prize to the top-ranked agent only, so when $F$ FOS dominates $H$, one might expect this to be the case as well. However, the example below illustrates that this is not true.
% The example below demonstrates that even if the target group agents have higher ability than the non-target group agents, it may be optimal to flatten the prize structure and distribute the budget to more than one top-ranked agents.
\footnote{In the preliminaries we assumed $F$ to be continuous, strictly increasing, and differentiable in $[0,1]$. In the following and the subsequent examples, the distribution $F$ is continuous but may not be strictly increasing and differentiable everywhere. If $F$ is not strictly increasing, we can add a slight gradient to resolve the issue; on the other hand, we can smooth out the finite number of points where it is not differentiable. These changes will have a minimal effect on the objective value and our analysis holds. For ease of presentation, we shall not discuss these issues.}

\begin{example}\label{ex:des:2}
Let $\mu = 1/8$, $F(x) = 1 - S(x)$, $G(x) = (x-\mu F(x))/(1-\mu)$, where $S(x)$ is given by:
\[
    S(x) = \begin{cases} 1, &\text{ if $x < 3/4$} \\
    16(1-x)^2, &\text{ if $3/4 \le x < 15/16$} \\
    1-x, &\text{ if $x \ge 15/16$}
    \end{cases}.
\]
It can be verified that $F(x)$ and $G(x)$ are continuous cumulative distribution functions. The distribution of the general population is $H(x) = \mu F(x) + (1-\mu) G(x) = x$. Also, $F(x) \le H(x)$ for every $x$ (and strict for some values of $x$), and therefore, $F$ FOS dominates $H$. The objective value is:
\begin{align*}
    &\frac{1}{j} \left( \int_0^{3/4} x f^H_{n-1,j}(x) dx \right. \\
    & \quad + \int_{3/4}^{15/16} 16x(1-x)^2 f^H_{n-1,j}(x) dx \\
    & \quad \left. + \int_{15/16}^1 x(1-x) f^H_{n-1,j}(x) dx \right) \\
    =& \ \frac{n-j}{j \cdot n} F^H_{n,j}\left(3/4\right)\\
    +& \frac{16(n-j)(j+1)}{n(n+1)(n+2)} (F^H_{n+2,j+2}(15/16) - F^H_{n+2,j+2}(3/4)) \\
    & \quad + \frac{n-j}{n(n+1)} \left(1-F^H_{n+1,j+1}\left(15/16\right)\right),
\end{align*}
where $F^H_{n,j}$ is the CDF corresponding to the PDF $f^H_{n,j}$.
% \begin{multline*}
%     = \frac{n-j}{j.n} F^H_{n,j}\left(3/4\right)\\
%     + \frac{16(n-j)(j+1)}{n(n+1)(n+2)} \left. (F^H_{n+2,j+2}\left(15/16\right) - F^H_{n+2,j+2}\left(3/4\right)\right. ) \\
%     + \frac{n-j}{n(n+1)} \left(1-F^H_{n+1,j+1}\left(15/16\right)\right).
% \end{multline*}
Note that $F^H_{n,j}$ is equal to the Beta distribution with parameters $n+1-j$ and $j$. The optimal value for $j$ may be derived with an involved calculation, but for our purpose, we just want to illustrate that the optimal $j$ is not $1$; it can be checked that for $n=50$, the optimal value for $j$ is $11$ and the optimal objective value is approximately $0.0498$.
\end{example}

Now we consider the case where $F$ and $H$ have the same mean but different variance, which implies second-order stochastic (SOS) dominance. The distribution with lower variance SOS dominates the one with higher variance, assuming both distributions have the same mean. The results are similar to FOS dominance: it may be optimal to have multiple prizes irrespective of whether $F$ or $H$ has a higher variance, as shown in the following examples. Note that FOS dominance implies SOS dominance, but not vice-versa.

\begin{example}
Let $\mu = 2/3$, $F(x) = 3x^2 - 2x^3$, and $G(x) = 3x - 6x^2 + 4x^3$. Observe that $H(x) = \mu F(x) + (1-\mu) G(x) = x$, and the variance of $H$ is $1/12$ while the variance of $F$ is $1/20$, and both have mean $1/2$. The objective value is given by:
\begin{multline*}
    \frac{1}{j} \int_0^1 x(1-3x^2+2x^3) f^H_{n-1,j}(x) dx \\
     = \frac{n-j}{j\cdot n} \left( 1 - \frac{(n+1-j)(n+2-j)}{(n+1)(n+2)} \right. \\
    \left. \left(3 - 2 \cdot \frac{n+3-j}{n+3} \right) \right).
\end{multline*}
Solving for $j$, we get $j = \frac{5n}{6} - \frac{\sqrt{7n^2+30n+39}}{6}+\frac{1}{2}$; as $j$ is integer, either the floor or the ceiling of this number is optimal. For example, for $n=50$, the optimal value is $19$. 
\end{example}

\begin{example}
 Let $\mu = 1/4$, $F(x) = 1-S(x)$, and $G(x) = (x-\mu F(x))/(1-\mu)$, where $S(x)$ is given by:
\[
    S(x) = \begin{cases} 1-48x/31, &\text{ if $x < 31/96$} \\
    1/2, &\text{ if $31/96 \le x < 3/4$} \\
    8(1-x)^2, &\text{ if $3/4 \le x < 7/8$} \\
    1-x, &\text{ if $x \ge 7/8$}
    \end{cases}
\]
It can be checked that $F(x)$ and $G(x)$ are valid and for the distribution of the general population we have $H(x) = \mu F(x) + (1-\mu) G(x) = x$. It can also be checked that the mean of all the distributions is $1/2$, and the variance of $H$ is $1/12 \approx 0.083$ while the variance of $F$ is $6703/55296 \approx 0.121 > 1/12$. The objective value is:
\begin{align*}
    &\frac{1}{j} \left( \int_0^{31/96} x \left(1-\frac{48}{31}x\right) f^H_{n-1,j}(x) dx \right. \\
    &\qquad + \int_{31/96}^{3/4} x\cdot\frac{1}{2}\cdot f^H_{n-1,j}(x) dx \\
    &\qquad + \int_{3/4}^{7/8} x\cdot 8\cdot (1-x)^2 f^H_{n-1,j}(x) dx \\
    &\qquad \left. + \int_{7/8}^{1} x (1-x) f^H_{n-1,j}(x) dx \right) \\
    &= \frac{n-j}{2\cdot j\cdot n} \left(F^H_{n,j}\left(31/96\right) + F^H_{n,j}\left(3/4\right)\right) \\
    &\qquad - \frac{48(n-j)(n+1-j)}{31 \cdot j \cdot n \cdot (n+1)} F^H_{n+1,j}\left(31/96\right) \\
    &\quad+ \frac{8(n-j)(j+1)}{n(n+1)(n+2)} (F^H_{n+2,j+2}(7/8) - F^H_{n+2,j+2}(3/4)) \\
    & \qquad + \frac{n-j}{n(n+1)} \left(1-F^H_{n+1,j+1}\left(7/8\right)\right).
\end{align*}
Note that $F^H_{n,j}$ is the Beta distribution with parameters $n+1-j$ and $j$. %, and the optimal value for $j$ can be derived with some effort. For our purpose, we just want to illustrate that the optimal $j$ need not be $1$; it can be checked that 
For $n=50$, the optimal value for $j$ is $11$ and the optimal objective value is approximately $0.0249$.
\end{example}
























\subsection{Group-Specific Prizes Only}\label{sec:desTarget}
In this section, we study the optimal prize structure when the prizes are accessible to the target group only. This models situations when there are separate contests for the target and the non-target group (there can be a separate contest for only non-target group agents, this will not have any affect on the strategy of the target group agents). We see that the optimal contest allocates the entire prize budget to the first prize, i.e., gives a prize of $1$ to the top-ranked agent in the group (Theorem~\ref{thm:desTarget}). The proof of Theorem~\ref{thm:desTarget} extends the techniques used to provide a similar result for total output~\cite{glazer1988optimal,moldovanu2001optimal}.

\begin{theorem}\label{thm:desTarget}
The contest with group-specific prizes only that maximizes the output of the target group awards a prize of $1$ to the top-ranked agent and $0$ to others.
\end{theorem}
\begin{proof}
From the equilibrium characterization in Theorem~\ref{thm:eqTarget}, we have
\begin{align*}
    \alpha(v) &= \sum_{j \in [n-1]} (\omega_j - \omega_{j+1}) \int_0^v y f_{n-1,j}^{\mu F + (1-\mu)}(y) dy \\
    &= \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^v y f_{n-1,j}^{\mu F + (1-\mu)}(y) dy,
\end{align*}
where $\gamma_j = j(\omega_j - \omega_{j+1}) \ge 0$. 

Let $H(x) = (1-\mu) + \mu F(x)$. We have $h(x) = \mu f(x)$ for $x > 0$ and $(1-H(x)) = \mu(1-F(x))$. Let 
$$
H_{n,j}(x) = \sum_{\ell = 0}^{j-1} \binom{n}{\ell} H(x)^{n-\ell} (1-H(x))^{\ell}
$$
be the distribution of the $j$-th highest order statistic of $H(x)$, and let $h_{n,j}(x)$ be its PDF, which is well-defined for $x > 0$, but at $x = 0$, $H_{n,j}(0)$ has a non-zero point mass. Note that $f_{n,j}^{\mu F + (1-\mu)}(x) = h_{n,j}(x)$.

The objective of the designer is $\bE_{v \sim F}[\alpha(v)]$
\begin{align*}
    &= \int_0^1 \left( \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^v y h_{n-1,j}(y) dy \right) dF(v) \\
    &= \sum_{j \in [n-1]} \gamma_j \frac{1}{j}  \int_0^1 y (1-F(y)) h_{n-1,j}(y) dy \\
    &= \sum_{j \in [n-1]} \gamma_j \frac{1}{\mu j}  \int_0^1 y (1-H(y)) h_{n-1,j}(y) dy \\ % \quad \text{ as $(1-H(x)) = \mu(1-F(x))$} \\
    &= \sum_{j \in [n-1]} \gamma_j \frac{1}{\mu n}  \int_0^1 y h_{n,j+1}(y) dy. % \quad \text{ as $(1-H(x)) h_{n-1,j}(x) = \frac{j}{n} h_{n,j+1}(x)$}.
\end{align*}
As $1/(\mu n)$ is a constant, to maximize the objective, the designer sets $\gamma_j > 0$ only for values of $j$ that maximize $\int_0^1 y h_{n,j+1}(y) dy$. From the definition of $H_{n,k}$, we have 
\begin{multline*}
    1 = H_{n,j+1}(1) = H_{n,j+1}(0) + \int_0^1 h_{n,j+1}(y) dy \\
        \implies \int_0^1 h_{n,j+1}(y) dy = 1 - H_{n,j+1}(0).
\end{multline*}
We also know that for any $x$ and $j < n$,
\begin{multline*}
    H_{n,j}(x) = \sum_{\ell = 0}^{j-1} \binom{n}{\ell} H(x)^{n-\ell} (1-H(x))^{\ell} \\
    \le \sum_{\ell = 0}^{j} \binom{n}{\ell} H(x)^{n-\ell} (1-H(x))^{\ell} = H_{n,j+1}(x).
\end{multline*}
Using this, we get
\begin{align}\label{eq:design:group:1}
    H_{n,1+1}(x) &\le H_{n,j+1}(x) \nonumber \\
    &\implies 1 - H_{n,2}(0) \ge 1 - H_{n,j+1}(0) \nonumber \\
    &\implies \int_0^1 h_{n,2}(y) dy \ge \int_0^1 h_{n,j+1}(y) dy,
\end{align}
for any $j \in [n-1]$. Observe that $h_{n,2}(y)$ is either \textit{single-crossing} with respect to $h_{n,j+1}(y)$, i.e., there is a point $x \in [0,1]$ s.t. $h_{n,2}(y) \le h_{n,j+1}(y)$ for $y \le x$ and $h_{n,2}(y) > f^H_{n,j+1}(y)$ for $y > x$, or $h_{n,2}(y)$ is always greater than $h_{n,j+1}(y)$, because
\begin{align*}
    \frac{h_{n,2}(y)}{h_{n,j+1}(y)} &= \frac{\binom{n-1}{1} H(y)^{n-2} (1-H(y))^{1} }{\binom{n-1}{j} H(y)^{n-j-1} (1-H(y))^{j}} \\
    &= \frac{(n-j-1)! j!}{(n-2)! (1-H(y))^{j-1}} \left( \frac{H(y)}{1-H(y)} \right)^{j-1},
\end{align*}
$\frac{H(y)}{1-H(y)}$ is strictly increasing and goes from $\frac{H(0)}{1-H(0)}$ to $\infty$ as $y$ goes to $1$, and the coefficient of $\frac{H(y)}{1-H(y)}$ is a constant. Using: (i) the identity function $y$ is an increasing function, (ii) $h_{n,2}(y)$ is single-crossing w.r.t. $h_{n,j+1}(y)$, and (iii) equation~(\ref{eq:design:group:1}), we have 
\begin{equation*}
    \int_0^1 y h_{n,2}(y) dy \ge \int_0^1 y h_{n,j+1}(y) dy.
\end{equation*}
So, it is optimal to only have a first prize.
\end{proof}



==> aaai/equilibrium.tex <==
\section{Equilibrium Analysis}\label{sec:eq}
In this section, we characterize the symmetric Bayes--Nash equilibrium (symmetric across the agents in a given group). We first solve for the equilibrium of the contest with both general and target group-specific prizes, then we specialize it to the two special cases: (1) general prizes only; (2) group-specific prizes only. 

\subsection{Both target group and general prizes}\label{sec:eqBoth}
\begin{theorem}\label{thm:eqBoth}
A contest with general prizes $(w_j)_{j \in [n]}$ and target group-specific prizes $(\omega_j)_{j \in [n]}$ has a Bayes--Nash equilibrium where an agent with ability $v \in [0,1]$ uses strategy $\alpha(v)$ if she is in the target group and strategy $\beta(v)$ if she is in the non-target group, where $\alpha(v)$ and $\beta(v)$ are defined as:
\begin{align*}
    \beta(v) &= \int_0^v (\mu f(k(y)) k'(y) + (1-\mu) g(y)) A(y) y d y,\\
    \alpha(v) &= \begin{cases} \beta(k^{-1}(v)), &\text{$0 \le v \le k(1)$} \\
                \int_{k(1)}^{v} \mu f(y) C(y) y dy, &\text{$k(1) \le v \le 1$}
                \end{cases},
\end{align*}
where:
\begin{itemize}
    \item $k$ is a function defined over $[0,1]$ and is the solution to the following ordinary differential equation, with boundary condition $k(0) = 0$,
    \[
        k'(v)  = \frac{(1-\mu) g(v) (v - k(v))A(v)}{\mu f(k(v)) ( k(v)A(v) + k(v)B(v) - v A(v) )}.
    \]
    \item $A(v) = \sum_{j \in [n]} w_j \psi(\mu F(k(v)) + (1-\mu) G(v))$.
    \item $B(v) = \sum_{j \in [n]} \omega_j \psi(\mu F(k(v)) + (1-\mu))$.
    \item $C(v) = \sum_{j \in [n]} (w_j + \omega_j) \psi(\mu F(v) + (1-\mu))$.
    \item $\psi(x) = \binom{n-1}{j-1} x^{n-j-1}(1-x)^{j-2} ( (n-j) - (n-1) x)$.
\end{itemize}
\end{theorem}
The proof is provided in the appendix. An important idea used in the proof is the function $k : [0,1] \rightarrow [0,1]$, which stands for $k(v) = \alpha^{-1}(\beta(v))$. Using $k$, we convert a pair of differential equations in $\alpha$ and $\beta$ that we get from the first-order equilibrium conditions to an ordinary differential equation in $k$, as given in the theorem statement. This technique is motivated by the work of \citet{amann1996asymmetric}, where they use to it analyze two-agent asymmetric contests.

If $F$ and $G$ are not \textit{simple} functions, then using Theorem~\ref{thm:eqBoth} to find analytical solutions for $\alpha$ and $\beta$ may not be tractable, so a numerical solution may have to be computed. 

% \abheek{this has mostly been resolved by the additional argument provided after the FOCs... the discontinuity of $\tilde{H}$ at $0$ is slightly problematic. My current justifying argument is: (1) the assumption that an agent with $0$ ability has $0$ output is reasonable because such an agent would have to put infinite effort to produce any output, which at most gets them a finite prize; (2) our assumption that for an agent with $v > 0$ has $\alpha(v) > 0$ and $\beta(v) > 0$ is consistent with the equations above, and (3) for such an agent the FOCs are satisfied by our solution, and the only place where the FOCs are not defined ($x=0$), we only need to show that the utility for the given strategy is positive, and therefore better than producing $x = 0$ output, which is missed by the FOCs.}

% \subsubsection*{Example: Equilibrium Analysis}
% Let there be only a prize of value $w$ accessible to all agents and a prize of value $\omega$ accessible to only target group agents. Let $F(x) = x^t$ and $G(x) = x^s$. We have $f(x) = t x^{t-1}$ and $g(x) = s x^{s-1}$.

% For this example, $A(v) = w A_1(v) = w (n-1) H(\beta(v))^{n-2} = w (n-1) (\mu k(v)^t + (1-\mu) v^s)^{n-2}$ and $B(v) = \omega B_1(v) = \omega (n-1) \tilde{\hat{H}}(\beta(v))^{n-2} = \omega (n-1) (\mu k(v)^t + (1-\mu))^{n-2}$. Replacing this in equation~(\ref{eq:sol:general:1}), and renaming $v$ by $x$ and $k(v)$ by $y$ to get a familiar differential equation formulation, we get
% \begin{equation*}
%     \frac{d y}{d x} = \frac{(1-\mu) s x^{s-1} (x - y) w (\mu y^t + (1-\mu) x^s)^{n-2}}{\mu t y^{t-1} ( y  \omega (\mu y^t + (1-\mu))^{n-2} - (x-y) w (\mu y^t + (1-\mu) x^s)^{n-2} )}
% \end{equation*}


\subsection{General Prizes Only}\label{sec:eqGen}
A contest designer may want to only award prizes that are equally accessible to all the agents. This model is particularly appealing for several real-life applications, because, although the design of the prize structure may incorporate distributional information about the ability of the agents in the two groups, the contest itself is completely unbiased. 

In our model, this design choice corresponds to setting $\omega_j = 0$ for all $j \in [n]$. For this case, the expected utility for a target group agent and a non-target group agent for a given pair of ability $v$ and output $b$ is the same. We can specialize the equilibrium characterization in Theorem~\ref{thm:eqBoth} to this case as follows:
\begin{theorem}\label{thm:eqGen}
A contest with general prizes only $(w_j)_{j \in [n]}$ has a Bayes--Nash equilibrium where an agent with ability $v \in [0,1]$ in the target or non-target group uses the strategy $\alpha(v)$, where $\alpha(v)$ is defined as:
\begin{equation*}
    \alpha(v) = \sum_{j \in [n-1]} (w_j - w_{j+1}) \int_0^v y f^{\mu F + (1-\mu) G}_{n-1,j}(y) dy.
\end{equation*}
\end{theorem}
This equilibrium is unique, as follows from a result by \citet{chawla2013auctions}. They prove that if a contest is anonymous (does not discriminate among the agents) and the abilities of the agents are sampled i.i.d. from a distribution, then the equilibrium is unique. With general prizes only, we can transform 
an instance of our problem (without changing its set of equilibria) to satisfy these requirements.


\subsection{Group-Specific Prizes Only}\label{sec:eqTarget}
In this case, there are no general prizes accessible to agents from both groups: all the prizes are allocated based on strict quotas for the groups. This model is similar to the model of seat quotas for college admissions studied by \citet{bodoh2018college}. Technically, in this case we assume that $w_j = 0$ for all $j \in [n]$. Here we focus on the target group; a similar result also holds for the non-target group, if there are any prizes reserved for them.
\begin{theorem}\label{thm:eqTarget}
A contest with target group-specific prizes only, $(\omega_j)_{j \in [n]}$, has a Bayes--Nash equilibrium where an agent with ability $v \in [0,1]$ in the target group uses strategy $\alpha(v)$, where $\alpha(v)$ is defined as:
\begin{equation*}
    \alpha(v) = \sum_{j \in [n-1]} (\omega_j - \omega_{j+1}) \int_0^v y f^{\mu F + (1-\mu)}_{n-1,j}(y) dy.
\end{equation*}
\end{theorem}

% The first order condition is:
% \begin{align*}
%     \alpha^{-1}(x) \sum_{j \in [n]} \omega_j \frac{d p^{\tilde{H}}_j(x)}{d x} = 1 \Longleftrightarrow v \sum_{j \in [n]} \omega_j C_j(v) \mu f(v) = \frac{d \alpha(v)}{d v},
% \end{align*}
% where $C_j(v) = \binom{n-1}{j-1} \tilde{H}(\alpha(v))^{n-j-1}(1-\tilde{H}(\alpha(v)))^{j-2} ( (n-j)(1-\tilde{H}(\alpha(v))) - (j-1)\tilde{H}(\alpha(v)) ) = B_j(\beta^{-1}(\alpha(v)))$, and because $\tilde{H}(\alpha(v)) = (1-\mu) + \mu F(v)$ and $\frac{d \tilde{H}(\alpha(v))}{d v} = \mu f(v)$ for $v > 0$. Further simplifying, we get:
% \begin{equation}\label{eq:sol:onlyGroup:1}
%     \alpha(v) = \sum_{j \in [n-1]} (\omega_j - \omega_{j+1}) \int_0^v y f_{n-1,j}^{\mu F + (1-\mu)}(y) dy.
% \end{equation}

==> aaai/intro.tex <==
\section{Introduction}
Contests---situations where multiple agents compete for valuable prizes---are prevalent in many real-life situations, including sports, R\&D races, crowdsourcing, college admissions (with both students competing for good universities and universities competing for good students) and job recruitment.\footnote{See the book by \citet{vojnovic2015contest} for an introduction to contest theory and relevant resources.} 

The dominant paradigm in contest theory is to assume that the principal designs the prize structure so as to incentivize the agents to produce a higher total output. In this model, the designer values the contribution from each agent equally, i.e., the marginal output produced by any agent contributes the same marginal value to the designer's objective. In this paper, we break away from this assumption: instead, we assume that the agents belong to two different groups and the designer may want to prioritize one group---the target group---over the other, non-target group.

Contests that give special importance to agents from a particular group are not uncommon in practice. Conferences give best student paper awards, in addition to best paper awards.\footnote{\url{https://aaai.org/Awards/paper.php}} Many competitions and hackathons are organized to elicit engagement from underrepresented groups: for example, recently Microsoft organized a hackathon as an intervention to get women interested in AI.\footnote{\url{https://news.microsoft.com/europe/features/bridging-the-stem-divide-ai-hackathon-helps-young-women-excel-in-computer-science/}} Similar prize allocation schemes can be observed, either directly or indirectly, in many other real-life situations, such as scholarship and internship allocation.

In this paper, we study an incomplete information (Bayesian) model. We assume that each agent is associated with an \textit{ability}, which captures the amount of output they can produce per unit effort. In an incomplete information model for contests, it is generally assumed that the abilities of the agents are selected i.i.d. from a given distribution $F$. In our model, based on the assumption that the agents belong to one of the two groups, the abilities of the agents in the target and the non-target group are sampled from 
two distinct distributions $F$ and $G$, respectively. Each agent belongs to the target group with a fixed probability $\mu$.
The agents know the prize allocation scheme, their own ability, and the prior distributions of other agents' abilities. They act strategically to maximize their expected utility, where the utility of an agent is the prize they receive minus the effort they exert, and reach a Bayes--Nash equilibrium. The contest designer knows the prior distributions of the agents' abilities; and therefore, can reason about the equilibrium behavior of the agents. She wants to design the prize allocation scheme so as to elicit equilibrium behavior that optimizes her own objective. We assume that the contest designer has a budget of $1$ to use for the prizes.

The contest ranks the agents based on their outputs, and awards the prizes based on the ranks. In our general model, we assume that contests have two sequences of prizes, one available to all agents, and the other available to the target group only. A conference sponsoring a best student paper award in addition to a best paper award is an example of such a contest. We also study two specific variants of this model. In the first variant, all prizes in the contest are equally accessible to all agents, and there are no group-specific prizes. One could come across such a design preference in situations where the contest designer does not want to discriminate among the agents, but still wants to incentivize an under-represented agent group. In this case, the contest does not discriminate while awarding the prizes, but the design of the prize structure (i.e., the value of the first prize, second prize, and so on) can incorporate the information about the ability distribution of the agents. This model captures an equal opportunity employer that treats all applicants equally, but has a preference to increase the diversity in the workplace. In the second variant, the contest has group-specific prizes only, with no prizes available to the entire population; examples include a hackathon for women in CS, or a hiring/scholarship contest with a strict group-specific quota.

We assume that the contest designer wants to maximize the expected output of the agents in the target group only. With minor changes, the techniques can be extended to an objective that maximizes the weighted sum of the group outputs and other similar objectives.

\subsection{Our Contribution}
We initiate a theoretical study of contest design to elicit higher participation by agents from under-represented groups, and propose tractable models to do so. We analyze the equilibrium behavior of the agents for three cases: \textit{general prizes only}, where there is a sequence of rank-ordered prizes accessible to all agents, whether in the target or the non-target group; \textit{group-specific prizes only}, where there are two different sequences of prizes, each accessible to one of the groups; \textit{both general and target group-specific prizes}, where there are prizes accessible to both groups as well as prizes accessible to the target group only. The techniques used to analyze the equilibrium in these contests can be extended to related prize structures.

Based on these equilibrium characterizations, we study the properties of the contest that maximizes the total expected output of the agents from the target group. For the setting where all prizes are general, we prove that the optimal contest awards a prize of $1/\ell$ to the first $\ell$ agents and $0$ to the remaining agents, where $\ell$ is a function of the relative frequency of target group agents, $\mu$, and the ability distributions of the target group, $F$, and the non-target group, $G$. We give a closed-form formula for $\ell$. We also study the effect of first-order and second-order stochastic dominance of $F$ on $G$, and vice versa, on the optimal contest. For the setting where all prizes are group-specific, we show that it is optimal to award the full prize of $1$ to the top-ranked agent, irrespective of the distributions $F$ and $G$. This result matches similar results on maximizing total output~\cite{moldovanu2001optimal}. We also compare general prizes and group-specific prizes, and show that either of these choices may be preferred depending upon the distributions $F$ and $G$, and also upon the frequency of the target group agents in the population, $\mu$, even if $F=G$.

% The contest designer cannot discriminate among the agents when awarding the prizes, but she may design the prizes to incentivize a particular group (we assume that the first group is the target group, with distribution $F$) to exert more effort, win more prizes, or have higher welfare.

% Why is this model relevant? In many real-world scenarios, contests are used as a mechanism to distribute resources (prizes) to achieve a broader goal, e.g., awarding scholarships, offering jobs, distributing funds to new small businesses, etc. Due to historical reasons, like differences in access to resources in the past, a particular group of agents may be less prepared to compete than others; but with more access to resources, these agents can improve and become more capable and better contributors to the society. Therefore, we may want to design the contest focusing on the welfare of such agents. In this paper, we ask whether this can be (partially) achieved keeping the contest anonymous, i.e., without directly using the group labels of the agents to assign prizes. In many situations, it may be necessary to keep the rules of the game same for every agent.

\subsection{Related Work}
We point the readers to the book by \citet{vojnovic2015contest} for a survey on contest theory.

\citet{glazer1988optimal} study a model with rank-order allocation of prizes, incomplete information with i.i.d. types sampled from a uniform distribution, and linear cost functions, and show that the contest that maximizes the total output awards the entire prize to the top-ranked agent. \citet{moldovanu2001optimal} characterize the symmetric Bayes--Nash equilibrium for a generalization of this model to any continuously differentiable distributions; \citet{chawla2013auctions} prove the uniqueness of this equilibrium. \citet{moldovanu2001optimal} also study non-linear cost functions and show that awarding the entire prize to the top-ranked agent is optimal when the agents have (weak) concave cost functions, but the optimal mechanism may have multiple prizes with convex cost functions. In contrast, we observe that even with linear cost functions, it may be beneficial to have multiple prizes to maximize the expected output from the target group. 

The standard assumption in mechanism design and its sub-area of contest design is that the agents' types are sampled i.i.d. from some distribution (see, e.g., \citet{myerson1981optimal} for auction design and \citet{moldovanu2001optimal} for contest design). Our paper extends the equilibrium analysis of \citet{moldovanu2001optimal} to an asymmetric model where the agents are from two groups with different distributions. \citet{amann1996asymmetric} study an asymmetric model with two agents with types sampled independently from two different distributions; our analysis uses the idea of the function `$k$' introduced by them, see Theorem~\ref{thm:eqBoth}. Characterizing equilibrium in contests with many agents with types sampled independently from different distributions has remained technically challenging; recently \citet{olszewski2016large, olszewski2020performance} made progress by assuming very large numbers of agents and prizes, where an individual agent has infinitesimal effect on the equilibrium.

\citet{bodoh2018college} model affirmative action in college admissions using contests. Their model has general non-linear utility and cost functions, but, like \citet{olszewski2016large, olszewski2020performance},
they assume that the numbers of agents and prizes are very large. They give first-order equilibrium conditions and show that two types of affirmative actions---(i) admissions preference schemes, where the outputs of agents from the target group are (artificially) amplified before ranking and prize allocation, and (ii) quotas, where there are separate pools of seats for the different groups
%, equivalent to our only group-specific prizes model (Section~\ref{sec:eqTarget})
---have the same sets of equilibria with identical actions by the agents and outcomes. Our model makes a stronger linearity assumption regarding the utility and cost functions, which allows us to better characterize the equilibrium and %also 
study the optimal contest (prize) design problem.

% Our paper focuses on multiple rank-order allocation prizes. 
There is a long line of literature on the effect of different types of affirmative actions on contests. This literature generally assumes that there is only one prize, which either gets allocated to the top-ranked agent or gets allocated proportionally (\citet{tullock1980efficient} contests and their generalizations), and the contest designer introduces different kinds of interventions in the allocation of this prize. One such intervention is \textit{favoritism}, where the objective is to maximize the total output by giving head-starts or handicaps to certain agents (see, e.g., \citet{kirkegaard2012favoritism,fu2020optimal,deng2021optimally}). A head-start (for weaker agents)
adds a bonus to an agent's output, while a handicap (for stronger agents) decreases an agent's score by a fixed percentage. See \citet{chowdhury2020heterogeneity} for a survey on contests and affirmative action.

% See the related work section of \citet{bodoh2018college} for a broader survey on affirmative action.

Our work deviates from the widely studied objective of maximizing total output, 
by focusing on the output of a target group. Several papers have studied objectives other than the total output, such as maximum individual output~\cite{chawla2019optimal}, cumulative output from the top $k$ agents~\cite{archak2009optimal,gavious2014revenue}, total output of agents producing output in a given range~\cite{elkind2021contest}. \citet{elkind2021contest}'s work targets agents based on their output level, and therefore, effectively, based on their abilities; our work targets agents based on their group association, with the assumption that exogenous factors may have caused agents in some groups to have acquired less ability.

There has also been extensive study in the complete information setting (e.g.,~\citet{baye1996all,barut1998symmetric,siegel2009all}). 
%We point the readers to the book by \citet{vojnovic2015contest} for a survey on contest theory. 



==> aaai/prelim.tex <==
\section{Model and Preliminaries}\label{sec:prelim}
Let there be $n$ agents. Any given agent belongs to the target (resp., non-target) group with probability $\mu$ (resp., $(1-\mu)$), independently of the other agents. Let $\bv = (v_1, v_2, \ldots, v_n)$ be the ability profile of the agents, where $v_i$ values are independent and identically distributed (i.i.d.) random variables from continuous and differentiable distributions $F$ or $G$ with support $[0,1]$, depending upon whether agent $i$ belongs to the target or the non-target group, respectively. Let $f$ and $g$ be the probability density functions (PDFs) of $F$ and $G$. The $n$ agents simultaneously produce the output profile $\bb = (b_i)_{i \in [n]}$, so that the cost of agent $i$ is $b_i/v_i$.

The contest awards two sequences of prizes $w_1 \ge w_2 \ge \ldots \ge w_n$ and $\omega_1 \ge \omega_2 \ge \ldots \ge \omega_n$, where the prize $w_j$ is given to the $j$-th ranked agent overall (we call these prizes \textit{general} prizes), and the prize $\omega_j$ is given to the $j$-th ranked agent among the agents in the target group (we call these \textit{group-specific} prizes), with ties broken uniformly. We assume that $\sum_j w_j + \sum_j \omega_j \le 1$, i.e., the contest designer has a unit budget. Given a vector of outputs $\bb$, let the allocation of general prizes be given by $\bx(\bb) = (x_{i,j}(\bb))_{i,j \in [n]}$, where $x_{i,j} = 1$ if agent $i$ is awarded the $j$-th prize and $x_{i,j} = 0$ otherwise. Similarly, let $\by(\bb,\bt) = (y_{i,j}(\bb,\bt))_{i,j \in [n]}$ be the allocation of target group prizes, where $\bt = (t_i)_{i \in [n]}$ is the group label vector; $t_i \in \{T,N\}$, $t_i = T$ if the agent is in the target group, $t_i = N$ if not. We shall suppress the notation for $\bt$ and write $\by(\bb)$ instead of $\by(\bb,\bt)$.

If agent $i$ is in the target group, her utility is given by:
\begin{multline}\label{eq:agentUtility1}
u_T(v_i, \bb, \bt) = \sum_{j \in [n]} w_j x_{i,j}(\bb) + \sum_{j \in [n]} \omega_j y_{i,j}(\bb) - b_i/v_i \\
\equiv v_i \left(\sum_{j \in [n]} w_j x_{i,j}(\bb) + \sum_{j \in [n]} \omega_j y_{i,j}(\bb)\right) - b_i,
\end{multline}
where the equivalence is true because scaling the utility function by a constant does not change the strategy of an agent. Similarly, the utility of an agent $i$ in the non-target group is given by:
\begin{equation}\label{eq:agentUtility2}
u_N(v_i, \bb, \bt) = v_i \sum_{j \in [n]} w_j x_{i,j}(\bb) - b_i.
\end{equation}

\subsection{Mathematical Preliminaries}
Let $p^H_j(v)$ denote the probability that a value $v \in [0, 1]$ is the $j$-th highest among $n$ i.i.d. samples from a distribution $H$, given by the expression:
\begin{equation*}
    p^H_j(v) = \binom{n-1}{j-1} H(v)^{n-j}(1-H(v))^{j-1}.
\end{equation*}

A key role in the Bayes--Nash equilibrium of rank-order allocation contests is played by the order statistics. Let $f^H_{n,j}$ be the PDF of the $j$-th highest order statistic out of $n$ i.i.d. samples from $H$ (with PDF $h$), given by the expression:
\begin{equation}\label{eq:OrderStat}
    f^H_{n,j}(v) = \frac{n!}{(j-1)!(n-j)!}H(v)^{n-j}(1-H(v))^{j-1}h(v).
\end{equation}
We shall also frequently use the following two identities for order statistics:
\begin{align*}
    H(v) f^H_{n-1,j}(v) &= \frac{n-j}{n} f^H_{n,j}(v);\\
    (1-H(v)) f^H_{n-1,j}(v) &= \frac{j}{n} f^H_{n,j+1}(v).
\end{align*}

\begin{definition}[(weak) first-order stochastic (FOS) dominance]\label{def:fosd}
A distribution $F$ {\em FOS dominates} another distribution $G$, if for every $x$, $F$ gives at least as high a probability of receiving at least $x$ as does $G$: $1-F(x) \ge 1-G(x) \Longleftrightarrow F(x) \le G(x)$.
\end{definition}

\begin{definition}[(weak) second-order stochastic (SOS) dominance]\label{def:sosd}
A distribution $F$ {\em SOS dominates} another distribution $G$, if for every $x$: $ \int_{-\infty}^x [F(t) - G(t)] dt \le 0$.
\end{definition}
FOS dominance implies SOS dominance. There is also another sufficient condition for SOS dominance: $F$ SOS dominates $G$ if $G$ is a mean-preserving spread of $F$.

Let us denote the inner product of two functions $\psi,\phi : [0,1] \rightarrow \bR_+$ by 
\[
    \langle \psi, \phi \rangle = \int_0^1 \psi(x) \phi(x) dx.
\]
When appropriately normalized, $\langle \psi, \phi \rangle$ measures the similarity between the functions $\psi$ and $\phi$.

% \paragraph{Mixture distribution.} Any given agent belongs to the first group with probability $\mu$, so her ability is selected from $F$ with probability $\mu$, and similarly, from $G$ with probability $(1-\mu)$. As the group and the ability of an agent is selected independently from other agents, so the ability $v$ of the agent is distributed by a mixture distribution $\mu F(v) + (1-\mu) G(v)$, with a PDF $\mu f(v) + (1-\mu) g(v)$.

\subsection{Equilibrium and Objective Function}
We shall study the Bayes--Nash equilibrium of the agents, where the agents in the target group use a symmetric strategy $\alpha(v)$ (symmetric across the agents in the group), where $\alpha(v)$ is the output of an agent with ability $v$; similarly, the agents in the non-target group use a symmetric strategy $\beta(v)$. The objective of the contest designer is to maximize the expected total output generated by the agents in the target group:
\begin{equation*}
    \sum_{i \in [n]} \bE_{v_i} [\alpha(v_i) \mid t_i = T] \bP[t_i = T] \equiv \bE_{v \sim F} [\alpha(v)]. %  = \mu \sum_{i \in [n]} \bE_{\bv} [\alpha(v_i)]
\end{equation*}

% \paragraph{Equilibrium behavior.} From the agents' perspective, the abilities of the agents are selected i.i.d. from a distribution $H$. \citet{moldovanu2001optimal} characterize the symmetric Bayes--Nash equilibrium for these contests. Chawla and Hartline~\cite{chawla2013auctions} prove the uniqueness of this equilibrium (see also \cite{chawla2019optimal}).

% \begin{theorem}(\cite{moldovanu2001optimal,chawla2013auctions})\label{thm:beta}
% Consider the game that models the rank-order allocation contest with the values of placement prizes $w_1 \ge w_2 \ge \ldots \ge w_n \ge 0$ and the abilities of the agents sampled i.i.d. from $H$. The unique Bayes--Nash equilibrium is given by
% \begin{equation}
%     \beta(v) = \sum_{j \in [n]} w_j \int_0^v t \frac{d p^H_j(t)}{dt} dt,
% \end{equation}
% where $\beta(v)$ is the output by an agent with valuation $v$. 
% \end{theorem}
% \noindent Note that $\beta$ is a function of $\bw$, but we are suppressing it to keep the notation cleaner. We shall use an equivalent formulation of the above equilibrium, used in \cite{elkind2021contest}:
% \begin{equation}\label{eq:betaS}
%     \beta(v) = \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^v t h_{n-1,j}(t) dt,
% \end{equation}
% where $\gamma_j = j (w_j - w_{j+1})$. Rather than optimizing over $(w_j)_{j \in [n]}$, one could optimize over $(\gamma_j)_{j \in [n-1]}$ with constraints $\gamma_j \ge 0$ and $\sum_j \gamma_j = 1$, to find the optimal contest that maximizes the designer's objective.

% % \paragraph{Expected Total (Group) Output.} If the designer wants to maximize the total expected output by all the agents, then the objective is $\bE_{v \sim H}[\beta(v)]$, but if she wants to maximize the output of the agents only in the first group, then the relevant objective is
% % \[ \bE_{v \sim F}[\beta(v)] = \int_0^1 \beta(v) dF(v) \]

% \abheek{To be continued... find the optimal contest with respect to the (1) total output, (2) social welfare, and (3) total prize, of the first group. Some preliminary analysis added below.}

==> ijcai-old/conclude.tex <==
\section{Conclusion}
% The development of underrepresented groups is integral to the progress of our society, and contests have been, and can be further, used to assist this goal. 
% Our work provides a theoretical framework to study such contests.
Our paper studies rank-order allocation prizes that aim to maximize the output of a target group. We provide equilibrium characterization for these contests and study the properties of the optimal contest.
For unbiased contests (i.e., with general prizes only), although it is preferable to award the prize to the top-performing player if the target group players are \textit{similar} to the overall population, if the target group players are very \textit{different}, then we may want to flatten out the prize structure. This does not only mean that we flatten out the prizes if the target group players are \textit{weaker} than others; we also demonstrate, if the target group players are \textit{stronger} but quite different than others, then also it may be a good idea to flatten out the prizes.
But for contests with fixed prize quotas (i.e., with group-specific prizes only), it may not be useful to flatten the prizes.
Regarding the choice between unbiased contests and fixed quota contests, the size of the target group in proportion to the size of the population plays an important role.

An important open problem is to understand the properties of the optimal contest that has both group-specific and general prizes. We characterize the equilibrium for this problem and analyze the optimal contest for specific sub-cases, but the general problem is open. One way to make this tractable may be to assume large numbers of agents and prizes; such assumptions allow for a stronger and more tractable equilibrium characterization by making the influence of an individual agent infinitesimal~\cite{olszewski2016large}. 
Our work focused on contests with a rank-order allocation of prizes with incomplete information and linear cost functions. %, but there are other good models to study contests that model real-life scenarios. For example, 
Instead of rank-order allocation of prizes, we can study a proportional allocation of prizes or its generalizations (see, e.g., \cite{tullock1980efficient}); one motivation for proportional allocation is the randomness and unpredictability of outcome in the real world. Similarly, we may relax the assumption of linear cost functions, or we can study complete information models instead of incomplete information.

\paragraph{Ethical Considerations}
There may be both short-term and long-term implications for designing contests specifically to incentivize a target group. For example, even if the contest itself is unbiased (Section \ref{sec:desGen}), optimizing the expected output of the players in the target group may mean that we decrease the expected total output of the entire population, and in particular decrease the expected total output of the non-target group. Moreover, such effects can be stronger if the target group forms a smaller fraction of the participants. Our analysis and examples try to capture such effects. For any given contest, this means that we are optimizing for the target group with a cost to society. But for a longer time frame, the answer is less obvious, and we believe that it is out of the scope of our paper. This question concerns whether practices like affirmative action have an overall positive or negative impact on our society in the long run. Our paper addresses the question: if we do want to use affirmative action in contests to incentivize the target group (with particular design choices, like the prize allocation scheme is unbiased), how to do it most effectively, and how it affects the output of all the players in the given contest.

==> ijcai-old/design.tex <==
\section{Designing Prizes to Incentivize the Target Group}\label{sec:des}
Based on the equilibrium characterizations in the previous section, in this section we investigate the properties of the optimal contest that maximizes the total output of the target group. We characterize the optimal contests for only general prizes and for only group-specific prizes.

% If the contest designer wants to have only general prizes, to induce maximum output from the target group, she should divide the prize budget equally among top-$k$ ranked agents, where $k$ depends upon the relative frequency of the target group agents $\mu$ and the distributions $F$ and $G$. This result is proved in Theorem~\ref{thm:desGen} and uses the equilibrium characterization given in Theorem~\ref{thm:eqGen}. 
% This result is in contrast to maximizing total output of the entire population, where the entire prize should be allocated to the top-ranked agent~\cite{glazer1988optimal,moldovanu2001optimal}.

% If the designer wants only group-specific prizes, she should allocate the entire prize budget to the first prize, i.e., give a prize of $1$ to the top-ranked agent in the group; given in Theorem~\ref{thm:desTarget}. The proof of Theorem~\ref{thm:desTarget} extends the techniques used to provide a similar result for total output maximization~\cite{glazer1988optimal,moldovanu2001optimal}.

In the appendix, we compare the choice between only general and only group-specific prizes; we observe that either of them may be a better choice depending upon the situation. Even if the distributions of the target and the non-target group are the same, the relative frequency of target group agents, measured by $\mu$, determines which prize allocation scheme is better. If $\mu$ is sufficiently high, then it is better to have only group-specific prizes, while the converse is true if $\mu$ is very low. 






\subsection{General Prizes Only}\label{sec:desGen}
The strategy used by the agents in the target group is $\alpha(v)$, as derived in Theorem~\ref{thm:eqGen}. It can be rewritten as
\begin{align}
    \alpha(v) &= \sum_{j \in [n-1]} (w_j - w_{j+1}) \int_0^v y f^{\mu F + (1-\mu) G}_{n-1,j}(y) dy \nonumber \\
    &= \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^v y f^{\mu F + (1-\mu) G}_{n-1,j}(y) dy,
\end{align}
where $\gamma_j = j (w_j - w_{j+1})$. Instead of optimizing over $(w_j)_{j \in [n]}$, we can optimize over $(\gamma_j)_{j \in [n-1]}$ with constraints $\gamma_j \ge 0$ and $\sum_j \gamma_j = 1$, to find the optimal contest that maximizes the target group's output.

\begin{theorem}\label{thm:desGen}
The contest with only general prizes that maximizes the expected total output of the agents in the target group awards a prize of $1/k^*$ to the $k^*$ top-ranked agents and a prize of $0$ to the remaining $n-k^*$ agents, where $k^*$ is defined as
\[
    k^* \in \argmax_{j \in [n-1]} \langle \psi , f^{\mu F + (1-\mu) G}_{n,j+1} \rangle
\]
for $\psi(x) = \frac{x (1-F(x))}{1- \mu F(x) - (1-\mu) G(x)}$.
\end{theorem}
\begin{proof} % [Proof of Theorem~\ref{thm:desGen}]
The expected output of an agent in the target group is $\bE_{v \sim F}[\alpha(v)]$, and maximizing this quantity maximizes the total output produced by all agents because $\mu$ and $n$ are constants. Let $H(v) = \mu F(v) + (1-\mu) G(v)$.
\begin{align*}
    &\bE_{v \sim F}[\alpha(v)] = \int_0^1 \alpha(v) dF(v) \\
    &= \int_0^1 \left( \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^v y f^{H}_{n-1,j}(y) dy \right) dF(v)\\
    &= \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^1 \left( \int_y^1 dF(v) \right) y f^{H}_{n-1,j}(y) dy \\ 
    &= \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^1 y (1-F(y)) f^{H}_{n-1,j}(y) dy. 
\end{align*}
As $\gamma_j \ge 0$ and $\sum_j \gamma_j = 1$, from the above expression we can observe that the optimal solution sets $\gamma_k > 0$ only if $\left(\frac{1}{j} \int_0^1 y (1-F(y)) f^{H}_{n-1,j}(y) dy \right)$ is maximized by $j = k$. Moreover, there is always an optimal solution where $\gamma_{k^*} = 1$ for some $k^* \in [n-1]$ and $\gamma_j = 0$ for $j \neq k^*$, where $k^*$ is given by:
\begin{align*}
    k^* &\in \argmax_{j \in [n-1]} \frac{1}{j} \int_0^1 y (1-F(y)) f^{H}_{n-1,j}(y) dy \\
    &= \argmax_{j \in [n-1]} \frac{1}{n} \int_0^1 y \frac{1-F(y)}{1-H(y)} f^{H}_{n,j+1}(y) dy \\
    &= \argmax_{j \in [n-1]} \langle \psi , f^{H}_{n,j+1}(y) \rangle,
\end{align*}
where $\psi(x) = x \frac{1-F(x)}{1-H(x)}$.
\end{proof}


Let $H(x)$ denote $\mu F(x) + (1-\mu) G(x)$. The function $\psi(x) = x\frac{1-F(x)}{1 - H(x)}$ in Theorem~\ref{thm:desGen} is independent of the prize structure: it depends only on $\mu$, $F$, and $G$, which are parameters given to the contest designer. The function $f^{H}_{n,j+1}(x)$ is the PDF of the $(j+1)$-th highest order statistic of the distribution $H$. The optimal $j = k^*$ maximizes the inner product between $\psi$ and $f^H_{n,j+1}$, and therefore, the similarity between them. In other words, the optimal $j = k^*$ selects the order statistic that is as similar to $\psi$ as possible.

Note that when we are maximizing the total output, then instead of an inner product of the order statistic with $\psi(x)$ in Theorem~\ref{thm:desGen}, we take an inner product with just $x$. As $x$ is monotonically increasing, the order statistic that is most similar to $x$ and that maximizes the inner product with $x$ is the one with $j = 1$, as shown by Moldovanu and Sela~\shortcite{moldovanu2001optimal}. This provides an argument in favor of allocating the entire prize budget to the first prize. In contrast, when we focus on the target group only, it may be optimal to distribute the prize among several top-ranked agents. This also means that we may lose a portion of the total output, and this loss can be $\Omega(n)$ as shown in Example~\ref{ex:des:0}. Also, by the \textit{single-crossing} property, see Vojnovic~\cite{vojnovic2015contest} Chapter 3, if we flatten the prize structure then we increase the output of the agents with low ability and decrease the output of the agents with high ability.

We have partially omitted calculations from the examples in this section. These examples are repeated in the appendix with more details. 

\begin{example}\label{ex:des:0}
Let $F(x) = 1 - (1-x)^{n-1}$, $G(x) = ((n-1)x - F(x))/(n-2)$, and $\mu = 1/(n-1)$. We get $H(x) = \mu F(x) + (1-\mu) G(x) = x$, which is the uniform distribution over $[0,1]$. Note that 
$\psi(x) = \frac{x(1-F(x))}{1-H(x)} = x(1-x)^{n-2}$.

It can be checked that the order-statistic that maximizes the inner-product with $\psi(x)$ is $f^H_{n,n-1}(x) = n(n-1)x(1-x)^{n-1}$. So, the optimal value is $k^* = n-2$. The total output generated for $k^* = n-2$ is $\frac{2}{n(n+1)}$.
On the other hand, we know that the expected total output is maximized by $j=1$ and is equal to $\frac{(n-1)}{n(n+1)}$.
The ratio between the two quantities is $(n-1)/2 = \Omega(n)$.
\end{example}


In the above example, the distribution of the target group $F$ was first-order stochastic (FOS) dominated by the distribution of the general population $H$.
% ; equivalently $F$ was FOS dominated by the distribution of the non-target group $G$. 
For this case, we observed that awarding prizes to more than one agent increases the expected output of the target group. $F$ being FOS dominated by $H$ means that the agents in the target group have lower ability than the general population. As flattening the prize structure increases the output of the lower ability agents and decreases the output of the higher ability agents, it makes sense that having a flatter prize structure incentivizes them.

The above result raises the question: What if the target group is equally able or stronger than the general population, i.e., if the distribution of the ability of an agent in the target group, $F$, FOS dominates the distribution of the ability of an agent in the non-target group, $G$; is it then optimal to award the prize to the top-ranked agent only? When $F = G = H$, we know that it is optimal to give prize to the top-ranked agent only, so when $F$ FOS dominates $H$, one might expect this to be the case as well. However, the example below illustrates that this is not true.
% The example below demonstrates that even if the target group agents have higher ability than the non-target group agents, it may be optimal to flatten the prize structure and distribute the budget to more than one top-ranked agents.
\footnote{In the preliminaries we assumed $F$ to be continuous, strictly increasing, and differentiable in $[0,1]$. In the following and the subsequent examples, the distribution $F$ is continuous and weakly increasing but may not be strictly increasing and differentiable everywhere. If $F$ is not strictly increasing, we can add a slight gradient to resolve the issue; on the other hand, we can smooth out the finite number of points where it is not differentiable. These changes will have a minimal effect on the objective value and our analysis holds. For ease of presentation, we shall not discuss these issues.}

\begin{example}\label{ex:des:2}
Let $\mu = 1/8$, $F(x) = 1 - S(x)$, $G(x) = (x-\mu F(x))/(1-\mu)$, where $S(x)$ is given by:
\[
    S(x) = \begin{cases} 1, &\text{ if $x < 3/4$} \\
    16(1-x)^2, &\text{ if $3/4 \le x < 15/16$} \\
    1-x, &\text{ if $x \ge 15/16$}
    \end{cases}.
\]
It can be verified that $F(x)$ and $G(x)$ are continuous cumulative distribution functions. The distribution of the general population is $H(x) = \mu F(x) + (1-\mu) G(x) = x$. Also, $F(x) \le H(x)$ for every $x$ (and strict for some values of $x$), and therefore, $F$ FOS dominates $H$. The optimal number of prizes $k^*$ need not be $1$; for example, for $n=50$, $k^* = 11$. 
\end{example}

Now we consider the case where $F$ and $H$ have the same mean but different variance, which implies second-order stochastic (SOS) dominance. The distribution with lower variance SOS dominates the one with higher variance, assuming both distributions have the same mean. The results are similar to FOS dominance: it may be optimal to have multiple prizes irrespective of whether $F$ or $H$ has a higher variance, as shown in the following examples. Note that FOS dominance implies SOS dominance, but not vice-versa.

\begin{example}\label{ex:des:3}
Let $\mu = 2/3$, $F(x) = 3x^2 - 2x^3$, and $G(x) = 3x - 6x^2 + 4x^3$. Observe that $H(x) = \mu F(x) + (1-\mu) G(x) = x$, and the variance of $H$ is $1/12$ while the variance of $F$ is $1/20$, and both have mean $1/2$.

Solving for $k^*$, we get $k^* = \frac{5n}{6} - \frac{\sqrt{7n^2+30n+39}}{6}+\frac{1}{2}$. For example, for $n=50$, $k^* = 19$.  
\end{example}

\begin{example}\label{ex:des:4}
 Let $\mu = 1/4$, $F(x) = 1-S(x)$, and $G(x) = (x-\mu F(x))/(1-\mu)$, where $S(x)$ is given by:
\[
    S(x) = \begin{cases} 1-48x/31, &\text{ if $x < 31/96$} \\
    1/2, &\text{ if $31/96 \le x < 3/4$} \\
    8(1-x)^2, &\text{ if $3/4 \le x < 7/8$} \\
    1-x, &\text{ if $x \ge 7/8$}
    \end{cases}
\]
It can be checked that $F(x)$ and $G(x)$ are valid and for the distribution of the general population we have $H(x) = \mu F(x) + (1-\mu) G(x) = x$. It can also be checked that the mean of all the distributions is $1/2$, and the variance of $H$ is $1/12 \approx 0.083$ while the variance of $F$ is $6703/55296 \approx 0.121 > 1/12$. The optimal number of prizes $k^*$ need not be $1$; for example, for $n=50$, $k^* = 11$. 
\end{example}
























\subsection{Group-Specific Prizes Only}\label{sec:desTarget}
In this section, we study the optimal prize structure when the prizes are accessible to the target group only. This models situations when there are separate contests for the target and the non-target group (there can be a separate contest for only non-target group agents, this will not have any affect on the strategy of the target group agents). We see that the optimal contest allocates the entire prize budget to the first prize, i.e., gives a prize of $1$ to the top-ranked agent in the group (Theorem~\ref{thm:desTarget}). The proof of Theorem~\ref{thm:desTarget} extends the techniques used to provide a similar result for total output~\cite{glazer1988optimal,moldovanu2001optimal}.

\begin{theorem}\label{thm:desTarget}
The contest with only group-specific prizes that maximizes the output of the target group awards a prize of $1$ to the top-ranked agent and $0$ to others.
\end{theorem}



==> ijcai-old/equilibrium.tex <==
\section{Equilibrium Analysis}\label{sec:eq}
In this section, we characterize the symmetric Bayes--Nash equilibrium (symmetric across the agents in a given group). We first solve for the equilibrium of the contest with both general and target group-specific prizes, then we specialize it for the two special cases: (1) only general prizes; (2) only group-specific prizes.

\subsection{Both Target Group and General Prizes}\label{sec:eqBoth}
\begin{theorem}\label{thm:eqBoth}
A contest with general prizes $(w_j)_{j \in [n]}$ and target group-specific prizes $(\omega_j)_{j \in [n]}$ has a Bayes--Nash equilibrium where an agent with ability $v \in [0,1]$ uses strategy $\alpha(v)$ if she is in the target group and strategy $\beta(v)$ if she is in the non-target group, where $\alpha(v)$ and $\beta(v)$ are defined as:
\begin{align*}
    \beta(v) &= \int_0^v (\mu f(k(y)) k'(y) + (1-\mu) g(y)) A(y) y d y,\\
    \alpha(v) &= \begin{cases} \beta(k^{-1}(v)), &\text{$0 \le v \le k(1)$} \\
                \int_{k(1)}^{v} \mu f(y) C(y) y dy, &\text{$k(1) \le v \le 1$}
                \end{cases},
\end{align*}
where:
\begin{itemize}
    \item $k$ is a function defined over $[0,1]$ and is the solution to the following ordinary differential equation, with boundary condition $k(0) = 0$,
    \[
        k'(v)  = \frac{(1-\mu) g(v) (v - k(v))A(v)}{\mu f(k(v)) ( k(v)A(v) + k(v)B(v) - v A(v) )}.
    \]
    \item $A(v) = \sum_{j \in [n]} w_j \psi(\mu F(k(v)) + (1-\mu) G(v))$.
    \item $B(v) = \sum_{j \in [n]} \omega_j \psi(\mu F(k(v)) + (1-\mu))$.
    \item $C(v) = \sum_{j \in [n]} (w_j + \omega_j) \psi(\mu F(v) + (1-\mu))$.
    \item $\psi(x) = \binom{n-1}{j-1} x^{n-j-1}(1-x)^{j-2} ( (n-j) - (n-1) x)$.
\end{itemize}
\end{theorem}
The proof is provided in the appendix. An important idea used in the proof is the function $k : [0,1] \rightarrow [0,1]$, which stands for $k(v) = \alpha^{-1}(\beta(v))$. Using $k$, we convert a pair of differential equations in $\alpha$ and $\beta$, which we get from the first-order equilibrium conditions, to an ordinary differential equation in $k$, as given in the theorem statement. This technique is motivated by the work of Amann and Leininger~\shortcite{amann1996asymmetric}, where they use to it analyze two-agent asymmetric contests.

If $F$ and $G$ are not \textit{simple} functions, then using Theorem~\ref{thm:eqBoth} to find analytical solutions for $\alpha$ and $\beta$ may not be tractable; a numerical solution may have to be computed. 

% \abheek{this has mostly been resolved by the additional argument provided after the FOCs... the discontinuity of $\tilde{H}$ at $0$ is slightly problematic. My current justifying argument is: (1) the assumption that an agent with $0$ ability has $0$ output is reasonable because such an agent would have to put infinite effort to produce any output, which at most gets them a finite prize; (2) our assumption that for an agent with $v > 0$ has $\alpha(v) > 0$ and $\beta(v) > 0$ is consistent with the equations above, and (3) for such an agent the FOCs are satisfied by our solution, and the only place where the FOCs are not defined ($x=0$), we only need to show that the utility for the given strategy is positive, and therefore better than producing $x = 0$ output, which is missed by the FOCs.}

% \subsubsection*{Example: Equilibrium Analysis}
% Let there be only a prize of value $w$ accessible to all agents and a prize of value $\omega$ accessible to only target group agents. Let $F(x) = x^t$ and $G(x) = x^s$. We have $f(x) = t x^{t-1}$ and $g(x) = s x^{s-1}$.

% For this example, $A(v) = w A_1(v) = w (n-1) H(\beta(v))^{n-2} = w (n-1) (\mu k(v)^t + (1-\mu) v^s)^{n-2}$ and $B(v) = \omega B_1(v) = \omega (n-1) \tilde{\hat{H}}(\beta(v))^{n-2} = \omega (n-1) (\mu k(v)^t + (1-\mu))^{n-2}$. Replacing this in equation~(\ref{eq:sol:general:1}), and renaming $v$ by $x$ and $k(v)$ by $y$ to get a familiar differential equation formulation, we get
% \begin{equation*}
%     \frac{d y}{d x} = \frac{(1-\mu) s x^{s-1} (x - y) w (\mu y^t + (1-\mu) x^s)^{n-2}}{\mu t y^{t-1} ( y  \omega (\mu y^t + (1-\mu))^{n-2} - (x-y) w (\mu y^t + (1-\mu) x^s)^{n-2} )}
% \end{equation*}


\subsection{General Prizes Only}\label{sec:eqGen}
A contest designer may want to only award prizes that are equally accessible to all the agents. This model is particularly appealing for several real-life applications, because, although the design of the prize structure may incorporate distributional information about the ability of the agents in the two groups, the contest itself is completely unbiased. 

In our model, this design choice corresponds to setting $\omega_j = 0$ for all $j \in [n]$. For this case, the expected utility for a target group agent and a non-target group agent for a given pair of ability $v$ and output $b$ is the same. We can specialize the equilibrium characterization in Theorem~\ref{thm:eqBoth} to this case as follows:
\begin{theorem}\label{thm:eqGen}
A contest with only general prizes $(w_j)_{j \in [n]}$ has a Bayes--Nash equilibrium where an agent with ability $v \in [0,1]$ in the target or non-target group uses the strategy $\alpha(v)$, where $\alpha(v)$ is defined as:
\begin{equation*}
    \alpha(v) = \sum_{j \in [n-1]} (w_j - w_{j+1}) \int_0^v y f^{\mu F + (1-\mu) G}_{n-1,j}(y) dy.
\end{equation*}
\end{theorem}
This equilibrium is unique, as follows from a result by Chawla and Hartline~\shortcite{chawla2013auctions}. They prove that if a contest is anonymous (does not discriminate among the agents) and the abilities of the agents are sampled i.i.d. from a distribution, then the equilibrium is unique. With only general prizes, we can transform 
an instance of our problem (without changing its set of equilibria) to satisfy these requirements.


\subsection{Group-Specific Prizes Only}\label{sec:eqTarget}
In this case, there are no general prizes accessible to agents from both groups: all the prizes are allocated based on strict quotas for the groups. This model is similar to the model of seat quotas for college admissions studied by bodoh-Creed and Hickman~\shortcite{bodoh2018college}. Technically, in this case we assume that $w_j = 0$ for all $j \in [n]$. Here we focus on the target group; a similar result also holds for the non-target group, if there are any prizes reserved for them.
\begin{theorem}\label{thm:eqTarget}
A contest with target only group-specific prizes, $(\omega_j)_{j \in [n]}$, has a Bayes--Nash equilibrium where an agent with ability $v \in [0,1]$ in the target group uses strategy $\alpha(v)$, where $\alpha(v)$ is defined as:
\begin{equation*}
    \alpha(v) = \sum_{j \in [n-1]} (\omega_j - \omega_{j+1}) \int_0^v y f^{\mu F + (1-\mu)}_{n-1,j}(y) dy.
\end{equation*}
\end{theorem}
Chawla and Hartline~\shortcite{chawla2013auctions}'s uniqueness result also applies to this equilibrium characterization, as it did for only general prizes, and for similar reasons (Section~\ref{sec:eqGen}).

% The first order condition is:
% \begin{align*}
%     \alpha^{-1}(x) \sum_{j \in [n]} \omega_j \frac{d p^{\tilde{H}}_j(x)}{d x} = 1 \Longleftrightarrow v \sum_{j \in [n]} \omega_j C_j(v) \mu f(v) = \frac{d \alpha(v)}{d v},
% \end{align*}
% where $C_j(v) = \binom{n-1}{j-1} \tilde{H}(\alpha(v))^{n-j-1}(1-\tilde{H}(\alpha(v)))^{j-2} ( (n-j)(1-\tilde{H}(\alpha(v))) - (j-1)\tilde{H}(\alpha(v)) ) = B_j(\beta^{-1}(\alpha(v)))$, and because $\tilde{H}(\alpha(v)) = (1-\mu) + \mu F(v)$ and $\frac{d \tilde{H}(\alpha(v))}{d v} = \mu f(v)$ for $v > 0$. Further simplifying, we get:
% \begin{equation}\label{eq:sol:onlyGroup:1}
%     \alpha(v) = \sum_{j \in [n-1]} (\omega_j - \omega_{j+1}) \int_0^v y f_{n-1,j}^{\mu F + (1-\mu)}(y) dy.
% \end{equation}

==> ijcai-old/intro.tex <==
\section{Introduction}
Contests---situations where multiple agents compete for valuable prizes---are prevalent in many real-life situations, including sports, R\&D races, crowdsourcing, college admissions and job recruitment.\footnote{See the book by Vojnovic~\shortcite{vojnovic2015contest} for an introduction to contest theory and relevant resources.} 

The dominant paradigm in contest theory is to assume that the principal designs the prize structure so as to incentivize the agents to produce a higher total output. In this model, the designer values the contribution from each agent equally, i.e., the marginal output produced by any agent contributes the same marginal value to the designer's objective. In this paper, we break away from this assumption: instead, we assume that the agents belong to two different groups and the designer may want to prioritize one group---the target group---over the other, non-target group.

Contests that give special importance to agents from a particular group are not uncommon in practice. Conferences give best student paper awards, in addition to best paper awards. %\footnote{\url{https://aaai.org/Awards/paper.php}} 
Many competitions and hackathons are organized to elicit engagement from underrepresented groups: for example, recently Microsoft organized a hackathon as an intervention to get women interested in AI.\footnote{\url{https://news.microsoft.com/europe/features/bridging-the-stem-divide-ai-hackathon-helps-young-women-excel-in-computer-science/}} Similar prize allocation schemes can be observed, either directly or indirectly, in many other real-life situations, such as scholarship and internship allocation.

In this paper, we study an incomplete information (Bayesian) model. We assume that each agent is associated with an \textit{ability}, which captures the amount of output they can produce per unit effort. In an incomplete information model for contests, it is generally assumed that the abilities of the agents are selected i.i.d. from a given distribution $F$. In our model, based on the assumption that the agents belong to one of the two groups, the abilities of the agents in the target and the non-target group are sampled from 
two distinct distributions $F$ and $G$, respectively. Each agent belongs to the target group with a fixed probability $\mu$.
The agents know the prize allocation scheme, their own ability, and the prior distributions of other agents' abilities. They act strategically to maximize their expected utility, where the utility of an agent is the prize they receive minus the effort they exert, and reach a Bayes--Nash equilibrium. The contest designer knows the prior distributions of the agents' abilities; therefore, can reason about the equilibrium behavior of the agents. She wants to design the prize allocation scheme so as to elicit equilibrium behavior that optimizes her own objective. We assume that the contest designer has a budget of $1$ to use for the prizes.

The contest ranks the agents based on their outputs and awards the prizes based on the ranks. In our general model, we assume that contests have two sequences of prizes, one available to all agents, and the other available to the target group only. A conference sponsoring a best student paper award in addition to a best paper award is an example of such a contest. We also study two specific variants of this model. In the first variant, all prizes in the contest are equally accessible to all agents, and there are no group-specific prizes. One could come across such a design preference in situations where the contest designer does not want to discriminate among the agents, but still wants to incentivize an under-represented agent group. In this case, the contest does not discriminate while awarding the prizes, but the design of the prize structure (i.e., the value of the first prize, second prize, and so on) can incorporate the information about the ability distribution of the agents. This model captures an equal opportunity employer that treats all applicants equally, but has a preference to increase the diversity in the workplace. In the second variant, the contest has group-specific prizes only, with no prizes available to the entire population; examples include a hackathon for women in CS, or a hiring/scholarship contest with a strict group-specific quota.

We assume that the contest designer wants to maximize the expected output of the agents in the target group only. With minor changes, the techniques can be extended to an objective that maximizes the weighted sum of the group outputs and other similar objectives.

\subsection{Our Contribution}
We initiate a theoretical study of contest design to elicit higher participation by agents from under-represented groups, and propose tractable models to do so. We analyze the equilibrium behavior of the agents for three cases: \textit{general prizes only}, where there is a sequence of rank-ordered prizes accessible to all agents, whether in the target or the non-target group; \textit{group-specific prizes only}, where there are two different sequences of prizes, each accessible to one of the groups; \textit{both general and target group-specific prizes}, where there are prizes accessible to both groups as well as prizes accessible to the target group only. The techniques used to analyze the equilibrium in these contests can be extended to related prize structures.

Based on these equilibrium characterizations, we study the properties of the contest that maximizes the total expected output of the agents from the target group. For the setting where all prizes are general, we prove that the optimal contest awards a prize of $1/\ell$ to the first $\ell$ agents and $0$ to the remaining agents, where $\ell$ is a function of the relative frequency of target group agents, $\mu$, and the ability distributions of the target group, $F$, and the non-target group, $G$. We give a closed-form formula for $\ell$. We also study the effect of first-order and second-order stochastic dominance of $F$ on $G$, and vice versa, on the optimal contest. For the setting where all prizes are group-specific, we show that it is optimal to award the full prize of $1$ to the top-ranked agent, irrespective of the distributions $F$ and $G$. This result matches similar results on maximizing total output~\cite{moldovanu2001optimal}. We also compare general prizes and group-specific prizes, and show that either of these choices may be preferred depending upon the distributions $F$ and $G$, and also upon the frequency of the target group agents in the population, $\mu$, even if $F=G$.

Omitted proofs are given in the appendix.

% The contest designer cannot discriminate among the agents when awarding the prizes, but she may design the prizes to incentivize a particular group (we assume that the first group is the target group, with distribution $F$) to exert more effort, win more prizes, or have higher welfare.

% Why is this model relevant? In many real-world scenarios, contests are used as a mechanism to distribute resources (prizes) to achieve a broader goal, e.g., awarding scholarships, offering jobs, distributing funds to new small businesses, etc. Due to historical reasons, like differences in access to resources in the past, a particular group of agents may be less prepared to compete than others; but with more access to resources, these agents can improve and become more capable and better contributors to the society. Therefore, we may want to design the contest focusing on the welfare of such agents. In this paper, we ask whether this can be (partially) achieved keeping the contest anonymous, i.e., without directly using the group labels of the agents to assign prizes. In many situations, it may be necessary to keep the rules of the game same for every agent.

\subsection{Related Work}
We discuss literature in contest theory directly relevant to our work; we point the readers to the book by Vojnovic~\shortcite{vojnovic2015contest} for a broader survey on contest theory.

Moldovanu and Sela~\shortcite{moldovanu2001optimal} characterize the Bayes--Nash equilibrium for contests with rank-order allocation of prizes assuming incomplete information with i.i.d. types; Chawla and Hartline~\shortcite{chawla2013auctions} prove the uniqueness of this equilibrium. Moldovanu and Sela~\shortcite{moldovanu2001optimal} also show that awarding the entire prize to the top-ranked agent is optimal when the agents have (weak) concave cost functions, but the optimal mechanism may have multiple prizes for convex cost functions. In contrast, we observe that even for linear cost functions, it may be beneficial to have multiple prizes to maximize the expected output from the target group. 

The standard assumption in mechanism design and its sub-area of contest design is that the agents' types are sampled i.i.d. from some distribution (see, e.g., \cite{myerson1981optimal} for auction design). Our paper extends the equilibrium analysis of Moldovanu and Sela~\shortcite{moldovanu2001optimal} to an asymmetric model where the agents are from two groups with different distributions. Amann and Leininger~\shortcite{amann1996asymmetric} study an asymmetric model with two agents with types sampled independently from two different distributions; our analysis uses the idea of the function `$k$' introduced by them, see Theorem~\ref{thm:eqBoth}. Characterizing equilibrium in contests with many agents with types sampled independently from different distributions has remained technically challenging; recently Olszewski and Siegel~\shortcite{olszewski2016large,olszewski2020performance} made progress by assuming very large numbers of agents and prizes, where an individual agent has infinitesimal effect on the equilibrium.

Bodoh-Creed and Hickman~\shortcite{bodoh2018college} model affirmative action in college admissions using contests. Their model has general non-linear utility and cost functions, but, like Olszewski and Siegel~\shortcite{olszewski2016large,olszewski2020performance},
they assume that the numbers of agents and prizes are very large. They give first-order equilibrium conditions and show that two types of affirmative actions---(i) admissions preference schemes, where the outputs of agents from the target group are (artificially) amplified before ranking and prize allocation, and (ii) quotas, where there are separate pools of seats for the different groups---have the same sets of equilibria with identical actions by the agents and identical outcomes. Our model makes a stronger linearity assumption regarding the utility and the cost functions, which allows us to better characterize the equilibrium and %also 
study the optimal contest (prize) design problem.

% Our paper focuses on multiple rank-order allocation prizes. 
There is a long line of literature on the effect of different types of affirmative actions on contests. This literature generally assumes that there is only one prize, which either gets allocated to the top-ranked agent or gets allocated proportionally (Tullock~\shortcite{tullock1980efficient} contests and their generalizations), and the contest designer introduces different kinds of interventions in the allocation of this prize. One such intervention is \textit{favoritism}, where the objective is to maximize the total output by giving head-starts or handicaps to certain agents (see, e.g., \cite{kirkegaard2012favoritism,fu2020optimal,deng2021optimally}). A head-start % (for weaker agents)
adds a bonus to an agent's output, while a handicap % (for stronger agents) 
decreases an agent's score by a fixed percentage. See \cite{chowdhury2020heterogeneity} for a survey on contests and affirmative action.

% See the related work section of t\cite{bodoh2018college} for a broader survey on affirmative action.

Our work deviates from the widely studied objective of maximizing total output, 
by focusing on the output of a target group. Several papers have studied objectives other than the total output, such as maximum individual output~\cite{chawla2019optimal}, cumulative output from the top $k$ agents~\cite{archak2009optimal,gavious2014revenue}, total output of agents producing output in a given range~\cite{elkind2021contest}. Elkind \textit{et al.}~\shortcite{elkind2021contest}'s work targets agents based on their output level, and therefore, effectively, based on their abilities; our work targets agents based on their group association, with the assumption that exogenous factors may have caused agents in some groups to have acquired less ability.

There has also been extensive study in the complete information setting (e.g.,~\cite{baye1996all,barut1998symmetric,siegel2009all}). 
%We point the readers to the book by \cite{vojnovic2015contest} for a survey on contest theory. 



==> ijcai-old/prelim.tex <==
\section{Model and Preliminaries}\label{sec:prelim}
Let there be $n$ agents. Any given agent belongs to the target (resp., non-target) group with probability $\mu$ (resp., $(1-\mu)$), independently of the other agents. Let $\bv = (v_1, v_2, \ldots, v_n)$ be the ability profile of the agents, where $v_i$ values are independent and identically distributed (i.i.d.) random variables from continuous and differentiable distributions $F$ or $G$ with support $[0,1]$, depending upon whether agent $i$ belongs to the target or the non-target group, respectively. Let $f$ and $g$ be the probability density functions (PDFs) of $F$ and $G$. The $n$ agents simultaneously produce the output profile $\bb = (b_i)_{i \in [n]}$, so that the cost of agent $i$ is $b_i/v_i$.

The contest awards two sequences of prizes $w_1 \ge w_2 \ge \ldots \ge w_n$ and $\omega_1 \ge \omega_2 \ge \ldots \ge \omega_n$, where the prize $w_j$ is given to the $j$-th ranked agent overall (we call these prizes \textit{general} prizes), and the prize $\omega_j$ is given to the $j$-th ranked agent among the agents in the target group (we call these \textit{group-specific} prizes), with ties broken uniformly. We assume that $\sum_j w_j + \sum_j \omega_j \le 1$, i.e., the contest designer has a unit budget. Given a vector of outputs $\bb$, let the allocation of general prizes be given by $\bx(\bb) = (x_{i,j}(\bb))_{i,j \in [n]}$, where $x_{i,j} = 1$ if agent $i$ is awarded the $j$-th prize and $x_{i,j} = 0$ otherwise. Similarly, let $\by(\bb,\bt) = (y_{i,j}(\bb,\bt))_{i,j \in [n]}$ be the allocation of target group prizes, where $\bt = (t_i)_{i \in [n]}$ is the group label vector; $t_i \in \{T,N\}$, $t_i = T$ if the agent is in the target group, $t_i = N$ if not. We shall suppress the notation for $\bt$ and write $\by(\bb)$ instead of $\by(\bb,\bt)$.

If agent $i$ is in the target group, her utility is given by
\begin{multline}\label{eq:agentUtility1}
u_T(v_i, \bb, \bt) = \sum_{j \in [n]} w_j x_{i,j}(\bb) + \sum_{j \in [n]} \omega_j y_{i,j}(\bb) - b_i/v_i \\
\equiv v_i \left(\sum_{j \in [n]} w_j x_{i,j}(\bb) + \sum_{j \in [n]} \omega_j y_{i,j}(\bb)\right) - b_i,
\end{multline}
where the equivalence is true because scaling the utility function by a constant does not change the strategy of an agent. Similarly, the utility of an agent $i$ in the non-target group is given by
\begin{equation}\label{eq:agentUtility2}
u_N(v_i, \bb, \bt) = v_i \sum_{j \in [n]} w_j x_{i,j}(\bb) - b_i.
\end{equation}

\subsection{Mathematical Preliminaries}
Let $p^H_j(v)$ denote the probability that a value $v \in [0, 1]$ is the $j$-th highest among $n$ i.i.d. samples from a distribution $H$, given by the expression
\begin{equation*}
    p^H_j(v) = \binom{n-1}{j-1} H(v)^{n-j}(1-H(v))^{j-1}.
\end{equation*}

A key role in the Bayes--Nash equilibrium of rank-order allocation contests is played by the order statistics. Let $f^H_{n,j}$ be the PDF of the $j$-th highest order statistic out of $n$ i.i.d. samples from $H$ (with PDF $h$), given by the expression
\begin{equation}\label{eq:OrderStat}
    f^H_{n,j}(v) = \frac{n!}{(j-1)!(n-j)!}H(v)^{n-j}(1-H(v))^{j-1}h(v).
\end{equation}
We shall also frequently use the following two identities for order statistics:
\begin{align*}
    H(v) f^H_{n-1,j}(v) &= \frac{n-j}{n} f^H_{n,j}(v);\\
    (1-H(v)) f^H_{n-1,j}(v) &= \frac{j}{n} f^H_{n,j+1}(v).
\end{align*}

\begin{definition}[(Weak) First-Order Stochastic (FOS) Dominance]\label{def:fosd}
A distribution $F$ {\em FOS dominates} another distribution $G$, if for every $x$, $F$ gives at least as high a probability of receiving at least $x$ as does $G$: $1-F(x) \ge 1-G(x) \Longleftrightarrow F(x) \le G(x)$.
\end{definition}

\begin{definition}[(Weak) Second-Order Stochastic (SOS) Dominance]\label{def:sosd}
A distribution $F$ {\em SOS dominates} another distribution $G$, if for every $x$: $ \int_{-\infty}^x [F(t) - G(t)] dt \le 0$.
\end{definition}
FOS dominance implies SOS dominance. Another sufficient condition for SOS dominance: $F$ SOS dominates $G$ if $G$ is a mean-preserving spread of $F$.

Let us denote the inner product of two functions $\psi,\phi : [0,1] \rightarrow \bR_+$ by 
\[
    \langle \psi, \phi \rangle = \int_0^1 \psi(x) \phi(x) dx.
\]
When appropriately normalized, $\langle \psi, \phi \rangle$ measures the similarity between the functions $\psi$ and $\phi$.

% \paragraph{Mixture distribution.} Any given agent belongs to the first group with probability $\mu$, so her ability is selected from $F$ with probability $\mu$, and similarly, from $G$ with probability $(1-\mu)$. As the group and the ability of an agent is selected independently from other agents, so the ability $v$ of the agent is distributed by a mixture distribution $\mu F(v) + (1-\mu) G(v)$, with a PDF $\mu f(v) + (1-\mu) g(v)$.

\subsection{Equilibrium and Objective Function}
We shall study the Bayes--Nash equilibrium of the agents, where the agents in the target group use a symmetric strategy $\alpha(v)$ (symmetric across the agents in the group), where $\alpha(v)$ is the output of an agent with ability $v$; similarly, the agents in the non-target group use a symmetric strategy $\beta(v)$. The objective of the contest designer is to maximize the expected total output generated by the agents in the target group:
\begin{equation*}
    \sum_{i \in [n]} \bE_{v_i \sim F} [\alpha(v_i) \mid t_i = T] \bP[t_i = T] \equiv \bE_{v \sim F} [\alpha(v)]. %  = \mu \sum_{i \in [n]} \bE_{\bv} [\alpha(v_i)]
\end{equation*}

% \paragraph{Equilibrium behavior.} From the agents' perspective, the abilities of the agents are selected i.i.d. from a distribution $H$. \cite{moldovanu2001optimal} characterize the symmetric Bayes--Nash equilibrium for these contests. Chawla and Hartline~\cite{chawla2013auctions} prove the uniqueness of this equilibrium (see also \cite{chawla2019optimal}).

% \begin{theorem}(\cite{moldovanu2001optimal,chawla2013auctions})\label{thm:beta}
% Consider the game that models the rank-order allocation contest with the values of placement prizes $w_1 \ge w_2 \ge \ldots \ge w_n \ge 0$ and the abilities of the agents sampled i.i.d. from $H$. The unique Bayes--Nash equilibrium is given by
% \begin{equation}
%     \beta(v) = \sum_{j \in [n]} w_j \int_0^v t \frac{d p^H_j(t)}{dt} dt,
% \end{equation}
% where $\beta(v)$ is the output by an agent with valuation $v$. 
% \end{theorem}
% \noindent Note that $\beta$ is a function of $\bw$, but we are suppressing it to keep the notation cleaner. We shall use an equivalent formulation of the above equilibrium, used in \cite{elkind2021contest}:
% \begin{equation}\label{eq:betaS}
%     \beta(v) = \sum_{j \in [n-1]} \gamma_j \frac{1}{j} \int_0^v t h_{n-1,j}(t) dt,
% \end{equation}
% where $\gamma_j = j (w_j - w_{j+1})$. Rather than optimizing over $(w_j)_{j \in [n]}$, one could optimize over $(\gamma_j)_{j \in [n-1]}$ with constraints $\gamma_j \ge 0$ and $\sum_j \gamma_j = 1$, to find the optimal contest that maximizes the designer's objective.

% % \paragraph{Expected Total (Group) Output.} If the designer wants to maximize the total expected output by all the agents, then the objective is $\bE_{v \sim H}[\beta(v)]$, but if she wants to maximize the output of the agents only in the first group, then the relevant objective is
% % \[ \bE_{v \sim F}[\beta(v)] = \int_0^1 \beta(v) dF(v) \]

% \abheek{To be continued... find the optimal contest with respect to the (1) total output, (2) social welfare, and (3) total prize, of the first group. Some preliminary analysis added below.}

==> ijcai-old/review/question.tex <==
Reviewer 1:
    1) Can you provide a quick explanation of the equilibria?
    
    2) What is the difficulty of extending the characterisation of the prizes to the setup with both group-specific and general prizes?
    
    3) Where does the definition of cost of an agent come from? What does it model?
    
    4) What is a good motivation to assume that mu is known?
    
    5) What does it mean exactly for ties to be broken arbitrarily? Why is this a good motivation? Usually in ranking contests, ties give rise to two "equal" prizes (as in e.g. Olympic Games).

Reviewer 2:
    1. Can you give an explanation of the statement in the proof of Theorem 4 that maximizing the expected output of an agent in the target group maximizes the total output of all agents. You have also mentioned that some portion of the total output may be lost for this purpose later?
    
    2. In Example 9, when we only have general prizes of value 1, should the expected target group output be non-zero with u = 0?
    
    3. If we only want to incentivize the output of the target group, why cannot we consider the group-specific prizes such that agents in non-target group have no incentives to participate?

    4. Example 1 shows that the loss of the total output can be Ω(n) when maximizing the output of the target group, will this value independent of F, G and u?
    
Reviewer 3:
    I'd like for the authors to address what they believe the work has to offer the field of AI.

==> old/additional.tex <==
\section{Additional Topics}
\abheek{These additional topics, like maximizing total effort or allocation of prizes to the target group, can be added if it seems relevant. Will take advise from Edith and Paul on what to do.}

\subsection{Maximizing Allocation of Prize to a Group}
In this section, we study the amount of prize that is allocated to the players in the first group. Note that $\beta(v)$ is a monotonically increasing function in $v$, so the ranking of the players is directly determined by their abilities. For the contest that awards the entire prize to the first ranked player, the expected amount of prize awarded to players in the first group is equal to the probability that the winner is in the first group. This probability can be computed as:
\begin{multline*}
    \bP[winner \sim F] = \sum_{i \in [n]} \bP[winner = i, i \sim F] = \sum_{i \in [n]} \bP[winner = i \mid i \sim F] \bP[i \sim F] \\
    = \alpha \sum_{i \in [n]} \bP[winner = i \mid i \sim F]
    % &= \alpha \sum_{i \in [n]} \int_0^1 H^{n-1}(v_i) dF(v_i) \\
    = \alpha n \int_0^1 H^{n-1}(v) dF(v),
\end{multline*}
where $i \sim F$ denotes player $i$ belongs to the first group (with distribution $F$).

In a similar manner, for a general rank-order prize allocation, we can compute the expected prize money awarded to players belonging to the first group as:
\begin{align*}
    \bE[\text{prize awarded to players $\sim F$}] &= \sum_{i \in [n]} \sum_{j \in [n]} w_j \bP[\text{player $i$ gets rank $j$}, i \sim F] \\
    &= \alpha \sum_{i \in [n]} \sum_{j \in [n]} w_j \bP[\text{player $i$ gets rank $j$} \mid i \sim F] \\
    &= \alpha n \sum_{j \in [n]} w_j \int_0^1 p^H_j(v) dF(v) \\
    &= \alpha n \sum_{j \in [n]} w_j \int_0^1 h_{n,j}(v) \frac{f(v)}{h(v)} dv. \\
\end{align*}
Note that we have assumed that the prizes are non-increasing $w_j \ge w_{j+1}$; this is essential to have an well-behaved equilibrium where the output $\beta(v)$ is monotonically increasing in ability.

From the analysis above, we see that the optimal contest if again a simple contest that distributes the prize among first $k$ players, where $k$ is given by:
\[ k = \argmax_{l \in [n]} \sum_{j \in [l]}\frac{1}{l} \int_0^1 h_{n,j}(v) \frac{f(v)}{h(v)} dv. \]

The extreme cases: if $\frac{f(v)}{h(v)}$ is an increasing function, then it is optimal to allocate the prize to the first-ranked player, because $\int_0^1 h_{n,j}(v) dv = 1$ for every $j$ and $h_{n,j}(v)$ is single-crossing w.r.t. $h_{n,l}(v)$ for $l > j$; if $\frac{f(v)}{h(v)}$ is a decreasing function, we should distribute the prize equally among all $n$ players, which leads to no competition and zero output from every player; if $\frac{f(v)}{h(v)} = constant$ (where $constant$ must be $1$), then any prize allocation scheme is equivalent as $\int_0^1 h_{n,j}(v) dv = 1$ for every $j$.

In general, the shapes of $h_{n,j}(v)$ and $\frac{f(v)}{h(v)}$ together determines the optimal contest, where $\int_0^1 h_{n,j}(v) \frac{f(v)}{h(v)} dv$ is the inner-product between the two functions, and therefore captures similarity between them. The function among $\left( \sum_{j \in [l]} \frac{1}{l} h_{n,j}(v) \right)_{l \in [n]}$ that is most similar to $\frac{f(v)}{h(v)}$ is selected.
